Efficient Constructions for the Gy\H{o}ri-Lov\'{a}sz Theorem on Almost Chordal Graphs

In the 1970s, Gy\H{o}ri and Lov\'{a}sz showed that for a $k$-connected $n$-vertex graph, a given set of terminal vertices $t_1, \dots, t_k$ and natural numbers $n_1, \dots, n_k$ satisfying $\sum_{i=1}^{k} n_i = n$, a connected vertex partition $S_1, \dots, S_k$ satisfying $t_i \in S_i$ and $|S_i| = n_i$ exists. However, polynomial algorithms to actually compute such partitions are known so far only for $k \leq 4$. This motivates us to take a new approach and constrain this problem to particular graph classes instead of restricting the values of $k$. More precisely, we consider $k$-connected chordal graphs and a broader class of graphs related to them. For the first, we give an algorithm with $O(n^2)$ running time that solves the problem exactly, and for the second, an algorithm with $O(n^4)$ running time that deviates on at most one vertex from the given required vertex partition sizes.

==> preamble.tex <==
%!TEX root = main.tex

\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{todonotes}
%%easier for makros
\usepackage{xparse}
\bibliographystyle{plainurl}
\usepackage{tikz}
\usetikzlibrary{calc}

\SetKwInput{KwInput}{Input}                
\SetKwInput{KwOutput}{Output} 

\def\oI{\overline{I}}
\def\C{\mathcal{C}}

\def\gyori{Gy\H{o}ri\xspace}
\def\lovasz{Lov\'{a}sz\xspace}
\newtheorem*{gl-theorem}{\gyori-\lovasz Theorem}

\newcommand{\davis}[1]{\todo[color=green!40]{#1}}
\newcommand{\davisin}[1]{\todo[inline,color=green!40]{#1}}
\newcommand{\katrin}[1]{\todo[inline,color=red!40]{#1}}
\newcommand{\katerina}[1]{\todo[color=blue!40]{#1}}
\newcommand{\ziena}[1]{\todo[color=yellow!40]{#1}}
\newcommand{\zienain}[1]{\todo[inline,color=yellow!40]{#1}}
\newcommand{\zienainT}[1]{\todo[inline,color=green!80]{#1}}


\def\glp{GL-Partition\xspace}
\def\glps{GL-Partitions\xspace}
\def\bigO{\mathcal{O}}
\def\wmax{w_{\mathit{max}}}
\def\compi{\overline{I}}
\def\ourclass{$\text{HHI}_4^2$-free\xspace}

\def\algChordalGL{\texttt{ChordalGL}\xspace}
\def\algChordalGLweighted{\texttt{WeightedChordalGL}\xspace}

